Detecting Neighborhood Gentrification at Scale via Street-level Visual Data

Neighborhood gentrification plays a significant role in shaping the social and economic well-being of both individuals and communities at large. While some efforts have been made to detect gentrification in cities, existing approaches rely mainly on estimated measures from survey data, require substantial work of human labeling, and are limited in characterizing the neighborhood as a whole. We propose a novel approach to detecting neighborhood gentrification at a large-scale based on the physical appearance of neighborhoods by incorporating historical street-level visual data. We show the effectiveness of the proposed method by comparing results from our approach with gentrification measures from previous literature and case studies. Our approach has the potential to supplement existing indicators of gentrification and become a valid resource for urban researchers and policy makers.

==> figure/case_archived/case1.tex <==
\begin{figure}[ht!]
  \centering
  \includegraphics[width=0.48\textwidth]{figure/case1.png} 
  \caption{Case study on Prescott, Oakland. }
  \label{fig:case1}
\end{figure}

==> figure/case_archived/case2.tex <==
\begin{figure}[ht!]
  \centering
  \includegraphics[width=0.48\textwidth]{figure/case2.png} 
  \caption{Case study on McClymonds, Oakland. }
  \label{fig:case2}
\end{figure}

==> figure/case_archived/case3.tex <==
\begin{figure}[ht!]
  \centering
  \includegraphics[width=0.48\textwidth]{figure/case3.png} 
  \caption{Case study on Beacon Hill, Seattle. }
  \label{fig:case3}
\end{figure}

==> figure/case_archived/case4.tex <==
\begin{figure}[ht!]
  \centering
  \includegraphics[width=0.48\textwidth]{figure/case4.png} 
  \caption{Case study on Lincoln Park, Denver. }
  \label{fig:case4}
\end{figure}

==> figure/weight.tex <==
\begin{figure}[ht!]
  \centering
  \includegraphics[width=0.48\textwidth]{figure/weight.png}
  \caption{Weight distribution comparison between gentrifying (shown in red) and non-gentrifying (shown in blue) neighborhoods. The horizontal axis is the index of each time-lapsed street view pair $t^{(i)}$ sorted by the value of weight $a_i$ in the descending order. The horizontal axis is the value of weight $a_i$. }
  \label{fig:weight}
\end{figure}
